Towards Exact Molecular Dynamics Simulations with Machine-Learned Force Fields

Molecular dynamics (MD) simulations employing classical force fields constitute the cornerstone of contemporary atomistic modeling in chemistry, biology, and materials science. However, the predictive power of these simulations is only as good as the underlying interatomic potential. Classical potentials often fail to faithfully capture key quantum effects in molecules and materials. Here we enable the direct construction of flexible molecular force fields from high-level ab initio calculations by incorporating spatial and temporal physical symmetries into a gradient-domain machine learning (sGDML) model in an automatic data-driven way. The developed sGDML approach faithfully reproduces global force fields at quantum-chemical CCSD(T) level of accuracy and allows converged molecular dynamics simulations with fully quantized electrons and nuclei. We present MD simulations, for flexible molecules with up to a few dozen atoms and provide insights into the dynamical behavior of these molecules. Our approach provides the key missing ingredient for achieving spectroscopic accuracy in molecular simulations.

==> ccsd_model_table.tex <==
%
\begin{table}[h!]
\caption{Prediction accuracy for interatomic forces and total energies of the sGDML$@$CCSD(T) model on all datasets. Energy errors are in kcal $\text{mol}^{-1}$, force errors in kcal $\text{mol}^{-1} \text{\AA}^{-1}$.}
\begin{threeparttable}
\label{tab:ccsd_results}
\setlength\extrarowheight{1pt}
\begin{ruledtabular}
\begin{tabular}{llrrrrrrrr}
\multicolumn{2}{l}{Dataset} & \multicolumn{2}{l}{Energy Prediction} & \multicolumn{3}{l}{Force Prediction}\\[2pt]
\cline{1-2} \cline{3-4} \cline{5-10}
\\ [-2.3ex]
&&&&&&\multicolumn{2}{l}{Magnitude} & \multicolumn{2}{l}{Angle} \\[2pt]
\cline{7-8} \cline{9-10}
 \\ [-2.3ex]
Molecule & \# ref. & MAE & RMSE & MAE & RMSE & MAE & RMSE & MAE & RMSE \\[1pt]
\hline \\ [-2.3ex]
Benzene & % 40, e-15, 28, ref MAE F: 0.2321, E: 0.070562
\ensuremath{1000} &
\ensuremath{0.004} &
\ensuremath{0.005} &
\ensuremath{0.04} &
\ensuremath{0.06} &
\ensuremath{0.04} &
\ensuremath{0.06} &
\ensuremath{0.0008} &
\ensuremath{0.0013}\\
Aspirin* & % 1000, e-15, 68
\ensuremath{1000} &
\ensuremath{0.16} &
\ensuremath{0.21} &
\ensuremath{0.76} &
\ensuremath{1.07} &
\ensuremath{0.56} &
\ensuremath{0.74} &
\ensuremath{0.0091} &
\ensuremath{0.0123}\\
Malonaldehyde & % 200, e-15, 10 (reduced) / 1000, e-15, 58 (full)
\ensuremath{1000} &
\ensuremath{0.06} &
\ensuremath{0.08} &
\ensuremath{0.37} &
\ensuremath{0.56} &
\ensuremath{0.34} &
\ensuremath{0.46} &
\ensuremath{0.0052} &
\ensuremath{0.0082}\\
Ethanol & % 1000, e-15, 76 % 135, e-15, 28
\ensuremath{1000} &
\ensuremath{0.05} &
\ensuremath{0.07} &
\ensuremath{0.35} &
\ensuremath{0.51} &
\ensuremath{0.47} &
\ensuremath{0.65} &
\ensuremath{0.0056} &
\ensuremath{0.0104}\\
Toluene & % 1000, e-15, 44  /  56 (non-optimal sampling), e-15, 42 /  511 (non-optimal sampling)
\ensuremath{1000} &
\ensuremath{0.03} &
\ensuremath{0.04} &
\ensuremath{0.21} &
\ensuremath{0.30} &
\ensuremath{0.19} &
\ensuremath{0.24} &
\ensuremath{0.0028} &
\ensuremath{0.0042}\\
\end{tabular}
\end{ruledtabular}
\begin{tablenotes}
      \item [*] CCSD
\end{tablenotes}
\end{threeparttable}
\end{table}
%

==> sym_model_table.tex <==
%
\begin{table}[h!]
\caption{Prediction accuracy for interatomic forces and total energies of the sGDML$@$DFT on all datasets. Energy errors are in kcal $\text{mol}^{-1}$, force errors in kcal $\text{mol}^{-1} \text{\AA}^{-1}$.}
\label{tab:results_all_sym}
\setlength\extrarowheight{1pt}
\begin{ruledtabular}
\begin{tabular}{llrrrrrrrr}
\multicolumn{2}{l}{Dataset} & \multicolumn{2}{l}{Energy Prediction} & \multicolumn{3}{l}{Force Prediction}\\[2pt]
\cline{1-2} \cline{3-4} \cline{5-10}
\\ [-2.3ex]
&&&&&&\multicolumn{2}{l}{Magnitude} & \multicolumn{2}{l}{Angle} \\[2pt]
\cline{7-8} \cline{9-10}
 \\ [-2.3ex]
Molecule & \# ref. & MAE & RMSE & MAE & RMSE & MAE & RMSE & MAE & RMSE \\[1pt]
\hline \\ [-2.3ex]
Benzene & % 1000, e-15, 8
\ensuremath{1000} &
\ensuremath{0.10} &
\ensuremath{0.12} &
\ensuremath{0.06} &
\ensuremath{0.09} &
\ensuremath{0.06} &
\ensuremath{0.09} &
\ensuremath{0.0009} &
\ensuremath{0.0017}\\
Uracil & % 1000, e-15, 32
\ensuremath{1000} &
\ensuremath{0.11} &
\ensuremath{0.14} &
\ensuremath{0.24} &
\ensuremath{0.37} &
\ensuremath{0.22} &
\ensuremath{0.31} &
\ensuremath{0.0039} &
\ensuremath{0.0064}\\
Naphthalene & % 1000, e-15, 38
\ensuremath{1000} &
\ensuremath{0.12} &
\ensuremath{0.15} &
\ensuremath{0.11} &
\ensuremath{0.17} &
\ensuremath{0.11} &
\ensuremath{0.15} &
\ensuremath{0.0016} &
\ensuremath{0.0026}\\
Aspirin & % 1000, e-15, 68
\ensuremath{1000} &
\ensuremath{0.19} &
\ensuremath{0.25} &
\ensuremath{0.68} &
\ensuremath{0.96} &
\ensuremath{0.52} &
\ensuremath{0.68} &
\ensuremath{0.0094} &
\ensuremath{0.0139}\\
Salicylic acid & % 1000, e-15, 38
\ensuremath{1000} &
\ensuremath{0.12} &
\ensuremath{0.15} &
\ensuremath{0.28} &
\ensuremath{0.44} &
\ensuremath{0.32} &
\ensuremath{0.45} &
\ensuremath{0.0038} &
\ensuremath{0.0064}\\
Malonaldehyde & % 1000, e-15, 58
\ensuremath{1000} &
\ensuremath{0.10} &
\ensuremath{0.13} &
\ensuremath{0.41} &
\ensuremath{0.62} &
\ensuremath{0.39} &
\ensuremath{0.56} &
\ensuremath{0.0055} &
\ensuremath{0.0087}\\
Ethanol & % 1000, e-15, 76
\ensuremath{1000} &
\ensuremath{0.07} &
\ensuremath{0.09} &
\ensuremath{0.33} &
\ensuremath{0.49} &
\ensuremath{0.46} &
\ensuremath{0.63} &
\ensuremath{0.0051} &
\ensuremath{0.0083}\\
Toluene & % 1000, e-15, 42
\ensuremath{1000} &
\ensuremath{0.10} &
\ensuremath{0.12} &
\ensuremath{0.14} &
\ensuremath{0.21} &
\ensuremath{0.14} &
\ensuremath{0.19} &
\ensuremath{0.0020} &
\ensuremath{0.0031}\\
Paracetamol & % 1000, e-15, 62
\ensuremath{1000} &
\ensuremath{0.15} &
\ensuremath{0.20} &
\ensuremath{0.49} &
\ensuremath{0.70} &
\ensuremath{0.60} &
\ensuremath{0.84} &
\ensuremath{0.0073} &
\ensuremath{0.0118}\\
Azobenzene & % 1000, e-15, 100
\ensuremath{1000} &
\ensuremath{0.09} &
\ensuremath{0.13} &
\ensuremath{0.41} &
\ensuremath{0.61} &
\ensuremath{0.49} &
\ensuremath{0.71} &
\ensuremath{0.0059} &
\ensuremath{0.0105}\\
\end{tabular}
\end{ruledtabular}
\end{table}
%
